Naive Feature Selection: a Nearly Tight Convex Relaxation for Sparse Naive Bayes

Due to its linear complexity, naive Bayes classification remains an attractive supervised learning method, especially in very large-scale settings. We propose a sparse version of naive Bayes, which can be used for feature selection. This leads to a combinatorial maximum-likelihood problem, for which we provide an exact solution in the case of binary data, or a bound in the multinomial case. We prove that our convex relaxation bounds becomes tight as the marginal contribution of additional features decreases, using a priori duality gap bounds dervied from the Shapley-Folkman theorem. We show how to produce primal solutions satisfying these bounds. Both binary and multinomial sparse models are solvable in time almost linear in problem size, representing a very small extra relative cost compared to the classical naive Bayes. Numerical experiments on text data show that the naive Bayes feature selection method is as statistically effective as state-of-the-art feature selection methods such as recursive feature elimination, $l_1$-penalized logistic regression and LASSO, while being orders of magnitude faster.

==> Experiments.tex <==
Here we plot all the results from the experiments section.
\section*{Amazon Data set}
\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/amzn_log_featselect.png}
    }
    \caption{Amazon Dataset. Stage 2: Logistic Regression.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/amzn_mnb_featselect.png}
    }
    \caption{Amazon Dataset. Stage 2: MNB.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/amzn_svm_featselect.png}
    }
    \caption{Amazon Dataset. Stage 2: SVM.}
\end{figure}


\section*{IMDB Data set}
\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/imdb_log_featselect.png}
    }
    \caption{IMDB Dataset. Stage 2: Logistic Regression.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/imdb_mnb_featselect.png}
    }
    \caption{IMDB Dataset. Stage 2: MNB.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/imdb_svm_featselect.png}
    }
    \caption{IMDB Dataset. Stage 2: SVM.}
\end{figure}


\section*{MPQA Data set}
\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/mpqa_log_featselect.png}
    }
    \caption{MPQA Dataset. Stage 2: Logistic Regression.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/mpqa_mnb_featselect.png}
    }
    \caption{MPQA Dataset. Stage 2: MNB.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/mpqa_svm_featselect.png}
    }
    \caption{MPQA Dataset. Stage 2: SVM.}
\end{figure}


\section*{SST2 Data set}
\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/sst2_log_featselect.png}
    }
    \caption{SST2 Dataset. Stage 2: Logistic Regression.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/sst2_mnb_featselect.png}
    }
    \caption{SST2 Dataset. Stage 2: MNB.}
\end{figure}

\begin{figure}[H]
    \vspace*{-0.5cm}
    \makebox[\linewidth]{
        \includegraphics[width=1.25\linewidth]{figures/sst2_svm_featselect.png}
    }
    \caption{SST2 Dataset. Stage 2: SVM.}
\end{figure}


